Unfairness Despite Awareness: Group-Fair Classification with Strategic Agents

The use of algorithmic decision making systems in domains which impact the financial, social, and political well-being of people has created a demand for these decision making systems to be "fair" under some accepted notion of equity. This demand has in turn inspired a large body of work focused on the development of fair learning algorithms which are then used in lieu of their conventional counterparts. Most analysis of such fair algorithms proceeds from the assumption that the people affected by the algorithmic decisions are represented as immutable feature vectors. However, strategic agents may possess both the ability and the incentive to manipulate this observed feature vector in order to attain a more favorable outcome. We explore the impact that strategic agent behavior could have on fair classifiers and derive conditions under which this behavior leads to fair classifiers becoming less fair than their conventional counterparts under the same measure of fairness that the fair classifier takes into account. These conditions are related to the the way in which the fair classifier remedies unfairness on the original unmanipulated data: fair classifiers which remedy unfairness by becoming more selective than their conventional counterparts are the ones that become less fair than their counterparts when agents are strategic. We further demonstrate that both the increased selectiveness of the fair classifier, and consequently the loss of fairness, arises when performing fair learning on domains in which the advantaged group is overrepresented in the region near (and on the beneficial side of) the decision boundary of conventional classifiers. Finally, we observe experimentally, using several datasets and learning methods, that this fairness reversal is common, and that our theoretical characterization of the fairness reversal conditions indeed holds in most such cases.

==> VerifyingUnfairness.tex <==
% \section{Complexity of Verifying Unfairness}
% \sd{The title is a little bit odd, since it's really about whether a fair classifier becomes more unfair, not verifying fairness. I'm also inclined to think we should push this to later and lead off with the next section and an example showing that manipulation can lead to lower fairness, since that's really the headline.}

% In this section we discuss the computational complexity of verifying whether or not a given \emph{fair} classifier $f_F$ will become less fair than its baseline counterpart $f_C$, under a given metric $\mathcal{M}$, when both are trained on the distribution $\D$ over $(G, \X, \Y)$ and agents are strategic.

% \begin{theorem}\label{thm:complex}
%     When $f_C$ and $f_F$ are linear, $h_X(\x)$ is uniform, it is \#P-hard to verify if for a given budget $c$
%     \begin{align*}
%         &\underset{(\x, y, g)\sim\D}{\mathbb{E}}[\PR\big(f_C(\x')|g=1\big) - \PR\big(f_C(\x')|g=0)\big)]\\
%         \leq~&\underset{(\x, y, g)\sim\D}{\mathbb{E}}[\PR\big(f_F(\x')|g=1\big) - \PR\big(f_F(\x')|g=0)\big)]
%     \end{align*}
% \end{theorem}

% \begin{proof}
%     Note that the problem of computing the volume of a hypercube clipped by a hyperplane is \#P-hard.
%     Since $f_C$ and $f_F$ are linear their decision boundaries are equivalent to hyperplanes, and thus for the cost function $c(\x, \x') = ||\x - \x'||$, the decision boundaries of $f_C$ and $f_F$ are still also hyperplanes. If $\X=[0, 1]^n$ then computing the difference in positive rate between the two classifiers for a budget $B$ is equivalent to computing the volume of the $[0, 1]^d$ clipped by either hyperplane.
% \end{proof}

% Although for general distributions verifying the unfairness of a classifier is intractable, if we want to verify unfairness for a finite set of agents, say $\A \subset G\times\X\times\Y$ then the problem is solvable time  $\Theta\big(|\A| T\big)$, where $T$ is the time complexity of attacking the classifier. For linear classifiers this indicates that checking fairness can is achivable in time $\Theta\big(|\A|\big)$.
% \textcolor{red}{(Andrew: Should we explicitly state the attack for linear classifiers, my understating is that this fact is common knowledge?)}
%     Suppose that $\X = [0, 1]^d$, and that both $f_C$ and $f_F$ are linear decision rules, i.e. ${f_C(\x) = \mathbb{I}[\w_C^T \x + b_C \geq 0]}$
%     and ${f_F(\x) = \mathbb{I}[\w_F^T \x + b_F \geq 0]}$.

%     For any $f(\x) = \w^T\x + b$, the optimal strategy for an agent with true type, $\x$ can be found via the following program:
%     \begin{align*}
%         \min_{\x'\in \R^d}&||\x-\x'||_2\\
%         &\text{s.t. }~\w^T\x \geq \theta
%     \end{align*}
%     which has an analytic solution namely,
%     \begin{align*}
%         \x^* = 
%         \begin{cases}
%         \x &\text{ if } \w^T\x + b \geq 0\\
%         \x - \frac{\w^T\x - b}{||\w||_2^2}\w &\text{ otherwise}
%         \end{cases}
%     \end{align*}
%     thus if $||\x^*|| \leq B$ the optimal response of an agent with type $\x$ is to play $\x^*$, and otherwise play $\x$.
    
%     \textcolor{red}{(Andrew): Although exactly computing the difference in unfairness is hard, we know that checking the relative fairness of a classifier $f$ when agents have budget $B$ can be approximated by sampling some agents from $\D$ and using an off-the-shelf attack (e.g. PDG) to compute the agents best response.}
    

==> model.tex <==
\section{Preliminaries}

    \begin{table*}[h!]
        \centering
        \begin{tabular}{||c|l||}
        \hline\hline
            Variable & Definition \\
            \hline\hline
            $G$ & set of possible groups ($G = \{0, 1\}$)\\
            \hline
            $\Y$ & set of possible lables ($\Y = \{0, 1\}$\\
            \hline
            $\X$ & domain of features\\
            \hline
            $\D$ & distribution over $G\times\X\times\Y$\\
            \hline
            $\M_{\D}$ & fairness metric w.r.t. to distribution $\D$ ($\M$ = PR, TPR, or FPR)\\
            \hline
            $f_C$ & most accurate classifier\\
            \hline
            $f_F$ & most accurate ``fair" classifier\\
            \hline
            $\D_{f}^{(B)}$ & the induced distribution when agents, with budget $B$, best respond to classifier $f$\\
            \hline
            $L_{\D}(f)$ & error of $f$ w.r.t. to $\D$\\
            \hline
            $U_{\D}(f)$ & difference in fairness, of $f$, between groups w.r.t. to $\D$\\
            \hline\hline
        \end{tabular}
        \caption{Notation Table}
        \label{tab:notation}
    \end{table*}
    Let $G\times\X\times\Y$ be be a domain of agents, where $G = \{0, 1\}$ indicates group membership, $\Y = \{0, 1\}$ indicates true label, and $\X$ is a the set of nonsensitive agent features.
    Agents are of the form $\mathbf{a} = (g, \x, y)$ with $g\in G$, $\x\in \X$, and $y\in \Y$.
    Let $\D$ be a distribution over $G\times\X\times\Y$ with pdf $h_{(g, \x, y)}$, (subscripts are dropped to indicate marginal pdfs, e.g. $h_{\x}$ is the pdf of $\x\in \X$).
    Assume all types in $\X$ are possible, i.e $h_{\x}(\x) > 0$ for all $\x\in \X$. \yl{the notation $h_{\x}(\x)$ reads a bit weird. Im assuming the $\x$ in the subscript is not really a changing argument. not sure the best way to fix but suggesting: $h_{\x}(\x') > 0$ for all $\x' \in \X$ or use $h_{\X}$}
    
    
    Let $f_C: \X \rightarrow \{0, 1\}$ be a baseline classifier, which is selected to have maximum expected accuracy. 
    \sd{What does the above statement mean precisely? Below it seems that these are being selected in an omniscient manner -- is that the intent?}
    Let ${f_F: \X \rightarrow \{0, 1\}}$ be a ``$\beta$-fair" classifier w.r.t. to a fairness metric $\M$ (e.g. $\M$ is PR, FPR, or TPR), which is selected to have maximum accuracy while having unfairness at most $\beta$. That is,
    \begin{align*}
        f_C = \text{argmin}_{f}&~1 - \mathbb{P}_{(\x, y)}\big(f(\x) = y\big)\\
        \\
        f_F = \text{argmin}_{f}&~1 - \mathbb{P}_{(\x, y)}\big(f(\x) = y\big)
        \\
        \text{s.t.}~\big|\mathbb{E}\big[&\M(G_1, f_F(\x), y) - \M(G_0, f_F(\x), y)\big]\big|\leq \beta
    \end{align*}
    For ease of analysis we also discuss $f_F$ in the equivalent terms of $\alpha$-fairness for $\alpha\in[0, 1]$, that is
    \begin{align*}
        f_F = \text{argmin}_{f}&~(1-\alpha)\big(1 - \mathbb{P}_{(\x, y)}\big(f(\x) = y\big)\big)\\
        & + \alpha\big|\mathbb{E}\big[\M(G_1, f_F(\x), y) - \M(G_0, f_F(\x), y)\big]\big|
    \end{align*}
     \yl{so came back here to the $\alpha$-fairness thing. I had a disconnection when thinking $f_F$ being less fair in the results below. the later results seem to rely on the value of $\alpha$, but does a larger $\alpha$ imply a smaller unfairness? This is a bit unclear to me since the fairness constraints transfer into soft ones. For the $\beta$-fair classifier, a larger $\beta$ returns a more accurate classifier since the constraint is looser, but I feel it is possible for this classifier to actually be more fair...I don't want to incur too mcuh of surgical changes at the moment but we can state an assumption saying we focus on some sort of montonic cases }
    An agent $\aj = (g, \x, y) \sim \D$ is capable of manipulating their features $\x$, to produce new features $\x'$. The \emph{cost} of this manipulation is given by $c(\x, \x') \geq 0$.  
    The utility of an agent with features $\x$ reporting $\x'$ to the classifier $f$ is given by
    \begin{align*}
        f(\x') - f(\x) - c(\x, \x')
    \end{align*}
    Agents' action space is the entire $\X$, and we assume all agents are rational and are utility maximizers. \yl{added this.}
    \sd{We should probably elaborate a little on the implications of this formulation -- can just say that we normalize the utility of being selected to 1, and therefore it would only make sense to manipulate if the cost changed the probability of selection enough}
    \yl{agree with Sanmay. We can probably say that since $ f(\x') - f(\x) \leq 1$, agent would not report a $\x'$ that has $c(\x, \x') \leq 1$.  }
    \yl{One more thing: when we measure the fairness on the new distribution, does changing $\x$ to $\x'$ change the true label $y$ too? or not? might want to clarify.}
    
    

==> new.tex <==


\section{Fairness Reversals}

We now formally define the concept of \emph{fairness reversals}: strategic agent behavior results in the fair classifier $f_F$ becoming less fair than the conventional classifier $f_C$.
\begin{definition}
\textbf{Fairness Reversal:} Given conventional and fair classifiers $f_C$ and $f_F$ with unfairness $U(f_F) < U(f_C)$, manipulation cost $c(\x, \x')$, and manipulation budget $B$, a \emph{fairness reversal} occurs if $U(f_F^{(c, B)} \geq U(f_C^{(c, B)}$, where $f_F^{(c, B)}, f_C^{(c, B)}$ are the resulting classifiers when agents best respond to $f_F, f_C$.
\end{definition}


Next we define two common families of cost functions, \emph{outcome monotonic} and \emph{feature monotonic} costs, where the former captures the notion that higher quality lies are more expensive, while the latter captures the notion that larger lies are more expensive.
\begin{definition}
\textbf{Outcome monotonic cost:}\cite{Milli18} A manipulation cost function $c(\x, \x')$ is said to be \emph{outcome monotonic} if, $c(\x, \x')$ is monotonically decreasing in $\Pb{y=1|\x}$ and monotonically increasing in $\Pb{y=1|\x'}$.
\end{definition}

\begin{definition}
    \textbf{Feature monotonic costs:} \cite{TODO} A manipulation cost function $c(\x, \x')$ is said to be \emph{feature monotonic} if $c(\x, \x')$ is monotonically increasing w.r.t. to $||\x - \x'||$
\end{definition}



\subsection{Fairness and Accuracy}
Empirically we observe a trade-off between unfairness and error: when strategic agent behavior leads to a fairness reversal, it also leads to an accuracy reversal.

To theoretically explain this empirical finding, we show that there is an inverse relationship between the the change in unfairness and change in error when agents are strategic. 


\begin{theorem}
    Given the fair classifier $f_F$, suppose agents best respond to $f_F$ according to cost function $c(\x, \x')$ and budget $B$, resulting in classifier $f_F^{(c, B)}$.
    The error of $f_F$ increases if and only if the unfairness of $f_F$ decreases, i.e.
    \begin{align*}
       \mathcal{L}(f_F) < \mathcal{L}(f_F)^{(c, B)} \iff U(f_F) > U(f_F^{(c, B)})
    \end{align*}
\end{theorem}

\begin{proof}

\end{proof}



==> unfinished.tex <==
\section{Speculation/ Idea}


One of the common ways in the literature to find fair classifiers is by optimizing a weighted sum of loss $L$ and unfairness $U$, i.e.
\begin{align*}
    \min_{f}~w_1 L(f) + w_2 U(f)
\end{align*}
Let  $f_F$ is the solution to this equation.


Typically one would expect a classifier's accuracy to decreases when agents are strategic, but I don't think people have a good perception of how fairness changes when agents are strategic, and as such one may expect the classifier to become more, or less fair, with equal probability. But we may be able to make an augment which shows that in general fairness must decrease when agents are strategic.

First, $f_F$ was selected for its optimally on a weighted function of loss and unfairness. 
Thus, if agents are strategic and the unfairness drops with little change to the loss (meaning the classifier is still useful as a predictor), then it could not have been the case that $f_F$ was optimal, but that $f_F$ was akin to something like a saddle point which was mistaken for a local minimum, and thus even the baseline fairness of our classifier was flawed.

Second, algorithms which are made to have equal FNR, FPR, or Equal Odds, between groups typically have higher overall rates FNR or FPR than their baseline counterparts. When switching form base to fair, rather than making less errors, a classifier made to have equal FNR will take borderline advantaged group members who score a 1 and push them slightly below the decision boundary, increasing that groups FNR. Similarly classifiers made to have equal FPR will take borderline disadvantaged members scoring a 0 and push them slightly above the decision boundary, increasing that groups FPR.
This means that a fair classifier (fair under FNR, FPR, or Equal Odds) will have more agents from the advantaged group who are slightly below the decision boundary than a base classifier. This set of agents, those slightly below the decision boundary, are the only ones able to strategically misreport their features to be classified as a 1.
Meaning that in any realistic case, there is a high chance that the advantaged group gains more positive labels when being strategic, compared to the disadvantaged group, even when the two groups have identical cost functions.







    
    
    
    
    
    
    \section{Linear Decision Rules}
    Suppose that $\X = \R^d$, and that both $f_C$ and $f_F$ are linear decision rules, i.e. ${f_C(\x) = \mathbb{I}[\w_C^T \x + b_C \geq 0]}$
    and ${f_F(\x) = \mathbb{I}[\w_F^T \x + b_F \geq 0]}$.
    
    
    \paragraph{Optimal Response:}
    For any $f(\x) = \w^T\x + b$, the optimal strategy for an agent with true type, $\x$ can be found via the following program:
    
    \begin{align*}
        \min_{\x'\in \R^d}&||\x-\x'||_2\\
        &\text{s.t.} \w^T\x + b\geq 0
    \end{align*}
    
    If the optimal solution to this program, say $\x^*$, yields positive utility, i.e. ${||\x-\x^*||_2 \leq \frac{1}{\lambda}}$, then the best strategy is to report $\x^*$, otherwise the best strategy is to report $\x$.
    
    This program has an analytic solution of,
    \begin{align*}
        \x^* = 
        \begin{cases}
        \x &\text{ if } \w^T\x + b \geq 0\\
        \x - \frac{\w^T\x - b}{||\w||_2^2}\w &\text{ otherwise}
        \end{cases}
    \end{align*}
    
    \paragraph{Measuring Fairness}
    From the above best response, we know that strategic behavior will only change the decisions of agents who have 
    \[ 
    0 < \bigg|\bigg|\frac{\w^T\x - b}{||\w||_2^2}\w\bigg|\bigg|_2 \leq \frac{1}{\lambda}
    \]
    Denote the set of such types as $S$. 
    
    Then if $f_C$ is $\alpha$-fair when agents are strategic, $f_C$ is $[(1-\gamma_C) \alpha + \gamma_C \alpha_{S_C}]$-fair
    where $\gamma_C$ is the fraction of agents in $S_C$ and $\alpha_S$ is the fairness of $f_C$ restricted to $S_C$.
    We can similarly define the fairness of $f_F$, as ${(1-\gamma_F) \beta + \gamma_F \beta_{S_F}}$.
    
    
    Thus we can outline the instances in which $f_C$ is more fair under strategic behavior than $f_F$.
    Namely any time that 
    \[
    (1-\gamma_C) \alpha + \gamma_C \alpha_{S_C} \leq (1-\gamma_F) \beta + \gamma_F \beta_{S_F}
    \]
    
    Which essentially amounts to having $\alpha_{S_C} < \beta_{S_F}$. Since in general $S_C$ and $S_F$ do not depend on one another, there are an infinite number of examples in which $f_C$ is more fair under strategic behaviour than $f_F$. Checking if a given pair of classifiers is an example of this, should be polynomial unless the distribution over agent types is hard to work with.
    
    \emph{More specifically, the way we define the expected values in Equation (1) can result in intractable cases. For example, when working with a  distribution over agent types, computing $\gamma$ (the size of $S$) and $\alpha_S$ (the fairness on $S$) would require the distribution's PDF to be integrated over $S$, which may not even be possible, let alone tractable.
    On the other-hand if we have a set of $n$ agents $D$(i.e. a dataset), then the expected values are a sums, rather than integrals, of at most $n$ terms, thus $\alpha_S$ and $\gamma$ are computable in linear time.}
    
    \paragraph{Extension to other classifiers}
    If the set of types predicted as a 1  can be written as a finite union of convex sets (e.g. decision trees, or piecewise linear functions) then the set of agent who can misreport their type to score a 1, i.e. $S$, can be expressed in simple terms and for the case of a dataset, rather than a distribution, we should be able to compute $\gamma$ and $\alpha_S$ in polynomial time.
    
    
    \paragraph{Recovering the original fairness of linear classifiers}
    The fairness of both $f_F$ and $f_C$ can be ``recovered" by simply decreasing their respective bias term. Namely, if for $f_F$ and $b_C$ are the original bias terms, changing the terms to $b_F' = b_f - \frac{1}{\lambda^2}$ and $b_C' = b_C - \frac{1}{\lambda^2}$ will cause $f_F$ and $f_C$ to make the same decisions under strategic behavior, as they did under truthful reporting.
